Respecting priorities versus respecting preferences in school choice: When is there a trade-off?

A classic trade-off that school districts face when deciding which matching algorithm to use is that it is not possible to always respect both priorities and preferences. The student-proposing deferred acceptance algorithm (DA) respects priorities but can lead to inefficient allocations. We identify a new condition on school choice markets under which DA is efficient. Our condition generalizes earlier conditions by placing restrictions on how preferences and priorities relate to one another only on the parts that are relevant for the assignment. Whenever there is a unique allocation that respects priorities, our condition captures all the environments for which DA is efficient. We show through stylized examples and simulations that our condition significantly expands the range of known environments for which DA is efficient. We also discuss how our condition sheds light on existing empirical findings.

==> fig1.tex <==
\tikzset{edge from parent/.style=
            {thick, draw, edge from parent fork right},
         every tree node/.style=
            {draw,minimum width=1in,text width=1.5in,align=center},
            every node/.style={scale=0.9}}
            
\begin{tikzpicture}[scale=1.1]
% Mu
    \node at (2,3) {$\mu$};
% Student nodes
    \node (i1) at (0,2) {$i_1$};
    \node (i2) at (1,2) {$i_2$};
    \node (i3) at (2,2) {$i_3$};
    \node (idots) at (3,2) {$\ldots$};
    \node (ik) at (4,2) {$i_k$};

% School nodes 
    \node (s1) at (0,0) {$s_{(1)}$};
    \node (s2) at (1,0) {$s_{(2)}$};
    \node (s3) at (2,0) {$s_{(3)}$};
    \node (sdots) at (3,0) {$\ldots$};
    \node (sk) at (4,0) {$s_{(k)}$};

% Lines and edges    
    \draw[-latex] (i1) -- (s1);
    \draw[-latex] (s1) -- (i2);
    \draw[-latex] (s2) -- (i3);
    \draw[-latex] (sdots) -- (ik);
    \draw[-latex,bend right] (sk) edge [out=240, in=240,looseness=1.6] (i1);

  \end{tikzpicture}


==> fig2.tex <==
\tikzset{edge from parent/.style=
            {thick, draw, edge from parent fork right},
         every tree node/.style=
            {draw,minimum width=1in,text width=1.5in,align=center},
            every node/.style={scale=0.9}}
            
\begin{tikzpicture}
% Mu
    \node at (2,3) {$\mu'$};
% Student nodes
    \node (i1) at (0,2) {$i_1$};
    \node (i2) at (1,2) {$i_2$};
    \node (i3) at (2,2) {$i_3$};
    \node (idots) at (3,2) {$\ldots$};
    \node (ik) at (4,2) {$i_k$};

% School nodes 
    \node (s1) at (0,0) {$s_{(k)}$};
    \node (s2) at (1,0) {$s_{(1)}$};
    \node (s3) at (2,0) {$s_{(2)}$};
    \node (sdots) at (3,0) {$\ldots$};
    \node (sk) at (4,0) {$s_{(k-1)}$};


  \end{tikzpicture}
